A Closed-Form Approximation of the Gaussian Noise Model in the Presence of Inter-Channel Stimulated Raman Scattering

An accurate, closed-form expression evaluating the nonlinear interference (NLI) power in coherent optical transmission systems in the presence of inter-channel stimulated Raman scattering (ISRS) is derived. The analytical result enables a rapid estimate of the signal-to-noise ratio (SNR) and avoids the need for integral evaluations and split-step simulations. The formula also provides new insight into the underlying parameter dependence of ISRS on the NLI. The proposed result is applicable for dispersion unmanaged, ultra-wideband transmission systems that use optical bandwidths of up to 15 THz. The accuracy of the closed-form expression is compared to numerical integration of the ISRS Gaussian Noise model and split-step simulations in a point-to-point transmission, as well as in a mesh optical network scenario.

==> figures/util_90_drop_80_pwrvar_1_ch_51_seed1.tex <==
\begin{figure}
\centering
\includegraphics[]{main-figure6}
\caption{The NLI coefficient of every fifth channel (i.e. a channel of interest) after six spans where interfering channels are continuously added and dropped along the transmission with a network utilization of 90\%. The results were obtained by numerical simulations and using the proposed closed-form approximation \eqref{eq:SPM_CF} and \eqref{eq:XPM_CF}.}
\label{fig:eta_network_90}
\end{figure}
